Precise Task Formalization Matters in Winograd Schema Evaluations

Performance on the Winograd Schema Challenge (WSC), a respected English commonsense reasoning benchmark, recently rocketed from chance accuracy to 89% on the SuperGLUE leaderboard, with relatively little corroborating evidence of a correspondingly large improvement in reasoning ability. We hypothesize that much of this improvement comes from recent changes in task formalization---the combination of input specification, loss function, and reuse of pretrained parameters---by users of the dataset, rather than improvements in the pretrained model's reasoning ability. We perform an ablation on two Winograd Schema datasets that interpolates between the formalizations used before and after this surge, and find (i) framing the task as multiple choice improves performance by 2-6 points and (ii) several additional techniques, including the reuse of a pretrained language modeling head, can mitigate the model's extreme sensitivity to hyperparameters. We urge future benchmark creators to impose additional structure to minimize the impact of formalization decisions on reported results.

==> writing/abstract.tex <==
\begin{abstract}
The Winograd Schema Challenge (WSC) \citep{levesque2011WSC} was presented as an alternative to the Turing Test as a commonsense reasoning benchmark. While large pre-trained transformer models have produced state-of-the-art results for WSC, they still fall short of human performance. Some methods have approached this threshold with scores jumping from 64.4\% to 89.0\% or higher on the SuperGLUE leaderboard. One common change in many of these high performing models is their task formalization. While there are many speculations on the impacts of this change in formalization, no empirical study has rigorously verified them. We perform an ablation study consisting of six formalizations of WSC and find that (1) using multiple choice in prediction and masked language modeling improves performance and (2) training with paired candidate and query noun phrases, focusing on hard examples, and using masked language modeling reduces the model's sensitivity to hyperparameters. 

% to understand (1) the task's sensitivity to formalization and (2) what components attribute to this difference in performance. We find that using RoBERTa and changing the task formalization from P-SPAN to MC-MLM improves performance. While multiple choice evaluation allows the model to achieve better top scores, we find deeper reasons that allow MC-MLM to better learn commonsense reasoning and conclude that this formalization is more than just a shallow trick.


\end{abstract}

==> writing/appendices.tex <==
\begin{appendices}
\section{Winogrande}
\label{appendix:A}

\begin{table}[h]
    \centering
    \resizebox{.45\textwidth}{!}{
    \begin{tabular}{l l l l}
        \toprule
        Formalization & Top & 3\textsuperscript{rd} Quartile & Difference\\
        \midrule
        MC-MLM          & 69.5\% & 67.5\% & 1.9\% \\
        MC-SENT         & 68.0\% & 53.1\% & 14.8\%\\
        MC-SENT-PAIR    & 66.4\% & 53.9\% & 12.5\%\\
        MC-SENT-PLOSS   & 54.5\% & 53.0\% & 1.6\% \\
        P-SENT          & 63.2\% & 50.4\% & 12.8\% \\
        P-SPAN          & 67.9\% & 65.9\% & 1.9\% \\
        \bottomrule
    \end{tabular}}
    % \caption{Statistics of validation accuracy. Difference is between top and 3\textsuperscript{rd} quartile values. Test results are from an ensemble of top 5 models.}
    \caption{Statistics of validation accuracy. Difference is between top and 3\textsuperscript{rd} quartile values.}
    \label{tab:stats}
\end{table}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/winogrande_violin.pdf}
    \caption{Boxplot of validation accuracy from 60 runs on WinoGrande. The red line marks the median number and higher edge of the rectangle marks the 3\textsuperscript{rd} quartile. The numbers indicate the 3\textsuperscript{rd} quartile values.}
    \label{fig:results}
\end{figure*}
\end{appendices}

==> writing/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
By using the same contextual embedding network and simply changing task formalization, we reaffirm that MC-MLM largely outperforms P-SPAN on WSC. We learn that having access to candidate NPs during inference alone improves the performance on WSC by a large margin. However, this shallow change only contributes to part of the improvement. We find deeper reasons behind MC formalizations that allow pre-trained transformers to better learn commonsense reasoning.

Our ablation study shows that training with paired candidate and query NPs, higher weighting of difficult edge examples, and reusing MLM from pre-training also benefit learning. Potentially expanding upon these ideas may lead to even better methods to learning commonsense reasoning tasks. We recommend that researchers provide all options while collecting Winograd-like datasets. 

% For future work, similar analysis will be applied to larger and less biased datasets like WinoGrande \citep{sakaguchi2019winogrande} to evaluate how these findings may extend to other Winograd-like data. Furthermore, comparing these results may provide additional insights to how these changes may contribute to learning commonsense reasoning. 

% We learn that having access to candidate NPs during inference alone improves the performance on WSC by a large margin. However, this only contributes to part of the improvement. There are deeper reasons behind mutiple choice formalizations that allow pre-trained transformers to better learn commonsense reasoning. So is multiple choice formatting of the Winograd Schema Challenge task just a shallow trick? In short, no. We recommend that researchers provide all options while collecting Winograd-like datasets. 

% Our ablation study shows that training with paired candidate and query NPs, weighting edge examples higher, and reusing MLM also benefits training. Potentially, expanding upon these ideas may lead to even better methods to learning commonsense reasoning tasks.

==> writing/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Implementation}
\label{sec:data}
Our code\footnote{*ANONYMIZED*} uses PyTorch \citep{paszke2019pytorch}, Huggingface Transformers \citep{wolf2019huggingface}, and FAIRSEQ \citep{ott2019fairseq}. All our experiments use pre-trained RoBERTa-large model. Following \citet{liu2019RoBERTa}, we use AdamW \cite{loshchilov2018adamw} optimizer with (0.9, 0.999) $\beta$'s and 0.001 weight decay. We use a linear learning rate scheduler with 6\% warm up steps. We evaluate over validation set every epoch, and early stop if the performance does not improve for 20 validations. We conduct a random hyperparameter search of 60 trials over the space of learning rate \{1e-5, 2e-5, 3e-5\}, number of epochs \{10, 20, 40\}, batch size \{8, 16, 32, 64\}, and random seeds.

\subsection{Data}
\label{sec:data}
We use WSC data from SuperGLUE\footnote{\url{https://super.gluebenchmark.com/tasks}\label{wsc}} and WinoGrande \citep{sakaguchi2019winogrande}. 
Each example in WSC consist of a sentence, a PRON span, and an NP span. Following \citep{liu2019RoBERTa} for MC-based formalizations, we mine candidate NPs with spaCy\footnote{\url{https://spacy.io/}}. We only keep one example from the group of examples that share the same sentence and PRON and only differ by query NP.

WinoGrande examples provide a sentence with two NP options.  In the sentence, an underscore is placed at the location of the PRON. When using asymmetrical formalizations like P-SENT, we duplicates each example into two and in turn make one of the option being the query NP, and the other being the candidate NP. In order to use P-SPAN formalization, we use the first appearance of query NP or candidate NP in the sentence as the NP span, and use the underscore as PRON span. Except for the special cases above, other formalization can be applied seamlessly to both data sets.


\begin{figure*}[t]
    \centering
    \subfloat[WSC]{
            \includegraphics[width=0.8\textwidth]{figures/wsc_violin.pdf}
            \label{subfig:wsc}
        }\hfill
    \subfloat[WinoGrande]{
            \includegraphics[width=0.8\textwidth]{figures/winogrande_violin.pdf}
            \label{subfig:wsc}
        }\hfill
    \caption{Boxplot of validation accuracy from 60 runs on WSC. The red line marks the median number and higher edge of the rectangle marks the 3\textsuperscript{rd} quartile. The numbers indicate the 3\textsuperscript{rd} quartile values.}
    \label{fig:results}
\end{figure*}

\begin{table}[t]
    \centering
    \resizebox{.45\textwidth}{!}{
    \begin{tabular}{l l l l l}
        \toprule
        Formalization & Top & 3\textsuperscript{rd} Quartile & Difference & Test\\
        \midrule
        MC-MLM          & 92.3\% & 86.1\% & 6.3\%  & 86.3\%\\
        MC-SENT         & 87.5\% & 82.7\% & 4.8\%  & \\
        MC-SENT-PAIR    & 87.5\% & 78.9\% & 8.7\%  & \\
        MC-SENT-PLOSS   & 86.5\% & 67.3\% & 19.2\% & 86.3\%\\
        P-SENT          & 77.9\% & 63.7\% & 14.2\% & 67.1\%\\
        P-SPAN          & 76.0\% & 65.4\% & 10.6\% & 80.1\%\\
        \bottomrule
    \end{tabular}}
    \caption{Statistics of validation accuracy. Difference is between top and 3\textsuperscript{rd} quartile values. Test results are from an ensemble of top 5 models.}
    % \caption{Statistics of validation accuracy. Difference is between top and 3\textsuperscript{rd} quartile values.}
    \label{tab:stats}
\end{table}

\subsection{WSC Results}
\label{sec:WSC results}
Figure \ref{fig:results} shows the validation accuracy from 60 runs of each formalization. We also include the majority class baseline and human performance. Table \ref{tab:stats} shows the max results, 3\textsuperscript{rd} quartile results, and the difference between them.

We first observe that most formalizations are sensitive to hyperparameter choices and random seeds. Across all formalizations, the gap between the top value and 3\textsuperscript{rd} quartile is fairly large with a minimum of 4.8\% (Table \ref{tab:stats}). 

Comparing 3\textsuperscript{rd} quartile values in Figure \ref{fig:results}, we see MC-MLM outperforms P-SPAN on the validation set by 21.2\%. The largest improvement between MC-SENT-PLOSS and MC-SENT-PAIR of 10.8\% indicates paired training with both candidate and query NPs makes learning the task easier. The remaining 10.4\% increase is distributed  roughly evenly among the other changes in formalization, excluding P-SPAN to P-SENT.

When looking at the distribution of points, we see three main changes. First, including MC evaluation between P-SENT and MC-SENT-PLOSS extends the tail of higher scores and allows the model to achieve better accuracy. However, the body of both formalizations remains relatively unchanged suggesting that this may be due to favorable hyperparameters. We then see the tail of higher scores fattens between MC-SENT-PLOSS and MC-SENT-PAIR and ultimately becomes the body with MC-SENT. This suggests that paired training and scaling with softmax help the model more reliably achieve better performance. Finally, we see that the model achieves higher scores with less variance with the introduction of MLM between MC-SENT and MC-MLM. This may be a result of fine-tuning the existing MLM head rather than training a linear layer from scratch. 

\subsection{WinoGrande Results}
\label{sec:Winogrande results}

We run the experiments on the medium size Winogrande dataset and include the results in the Appendix \ref{appendix:A}. Similar to WSC, we observe MC-SENT-PAIR and MC-SENT incrementally making high performance easier to achieve, MC-MLM reducing the variance of the accuracy. However, there are two main differences. First, P-SPAN is much higher than its sentence-based counterpart P-SENT. We suspect this is because when collecting Winogrande, adversarial filtering deliberately removes examples easy to classify from sentence representation, while P-SPAN formalization bypass this since it does not rely on sentence representation. Second, the tail of higher scores are less common on Winogrande than WSC, this suggests Winogrande is more sensitive to hyperparameters and random seeds.

==> writing/intro.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, large pre-trained models \citep{devlin2018BERT} based on Transformer architecture \citep{vaswani2017transformer} have achieved super-human performance on natural language understanding (NLU) tasks. However, these models still fall short on the Winograd Schema Challenge (WSC) \citep{levesque2011WSC}. This task requires the reader to use contextual semantics to disambiguate pronoun reference. For example, in the sentence

\vspace{1mm}
\textit{``The trophy didn't fit into the brown suitcase because it was too small.''}
\vspace{1mm}

\noindent the reader must understand how a \textit{trophy} can fit into a \textit{suitcase} to determine the correct antecedent of the pronoun \textit{it}.

The path to human performance exhibits a dichotomy on the SuperGLUE \citep{wang2019superglue} leaderboard\footnote{\url{https://super.gluebenchmark.com/leaderboard}} with scores skyrocketing from 64.4\% to 89.0\% or higher. One common theme among high performing models \citep{liu2019RoBERTa} is a formalization of the task with masked language modeling (MLM). \citet{kocijan2019WSCTrick} show that using additional data and this formalization help BERT achieve an 8.8\% gain in performance. This begs the question how can changing formalization improve performance.

We refer to these two task formalizations as pointwise span (\textbf{P-SPAN}) and multiple choice masked language modeling (\textbf{MC-MLM}). P-SPAN uses a sigmoid span classifier to determine if the pronoun (PRON) refers to the noun phrase (NP) query. MC-MLM uses a softmax classifier to determine the reference of the masked PRON by comparing likelihoods among NP candidates. We investigate how reformatting WSC from P-SPAN to MC-MLM results in better performance. By comparing results from six formalizations, we seek to understand (1) the task's sensitivity to formalization and (2) what components contribute to MC-MLM's improved performance.

In this work, we reaffirm the impact of formalizations on WSC and find MC-MLM outperforms P-SPAN while both formalizations use the same contextual respresentations. From our ablation study, we find that MC-MLM's improvement is mainly due to multiple choice (MC) inference, paired training with query and candidate NPs, higher weighting of hard examples, and using an MLM head. While some of these components, like MC evaluation, may seem shallower in nature, we find deeper reasons that allow MC-MLM to better learn common sense reasoning in WSC.

==> writing/methodology.tex <==
% \begin{table*}[h]
%     \centering
%     \resizebox{.99\textwidth}{!}{
%     \begin{tabular}{p{.2\textwidth} p{1mm} p{.5\textwidth} l  p{.03\textwidth} p{.07\textwidth} p{.1\textwidth} p{.15\textwidth}}
%         \toprule
%         Formalization & & Input Example & Loss & MC & EMB & Label & Component\\
%         \midrule
%         \multirow{2}{*}{MC-MLM} & a) & \texttt{[CLS]} The \underline{trophy} didn't fit into the brown suitcase because \texttt{[MASK]} was too small. \texttt{[SEP]} & \multirow{2}{*}{$-\sum_i^n \delta_{y,i} \log \mathbb{P}(\text{NP}_i\vert \text{s})/\sum_j^n\mathbb{P}(\text{NP}_j\vert \text{s})$} & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\texttt{[MASK]}} & \multirow{2}{*}{Index} & \multirow{2}{*}{MLM} \\
%         & b) & \texttt{[CLS]} The trophy didn't fit into the brown \underline{suitcase} because \texttt{[MASK]} was too small. \texttt{[SEP]} & & & & & \\
%         \midrule
%         \multirow{2}{*}{MC-SENT} & a) & \texttt{[CLS]} The trophy didn't fit into the brown suitcase because trophy \texttt{[SEP]} was too small. \texttt{[SEP]} & \multirow{2}{*}{$-\sum_i^n \delta_{y,i} \log \mathbb{P}(\text{NP}_i\vert \text{s}_1,\ldots, \text{s}_n)$} & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\texttt{[CLS]}} & \multirow{2}{*}{Index} & \multirow{2}{*}{Scaling} \\
%         & b) & \texttt{[CLS]} The trophy didn't fit into the brown suitcase because suitcase \texttt{[SEP]} was too small. \texttt{[SEP]} & & & & & \\
%         \midrule
%         \multirow{2}{*}{MC-SENT-PAIR} & a) & \texttt{[CLS]} The trophy didn't fit into the brown suitcase because trophy \texttt{[SEP]} was too small. \texttt{[SEP]} & \multirow{2}{*}{$-\sum_i^n \left[y_i \log \mathbb{P}(\text{True}\vert \text{s}_i) + (1-y_i) \log \mathbb{P}(\text{False}\vert \text{s}_i)\right]$} & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\texttt{[CLS]}} & \multirow{2}{*}{Binary} & \multirow{2}{*}{Paired Training}\\
%         & b) & \texttt{[CLS]} The trophy didn't fit into the brown suitcase because suitcase \texttt{[SEP]} was too small. \texttt{[SEP]} & & & & & \\
%         \midrule
%         \multirow{2}{*}{MC-SENT-PLOSS} & a) & \texttt{[CLS]} The trophy didn't fit into the brown suitcase because trophy \texttt{[SEP]} was too small. \texttt{[SEP]} & \multirow{2}{*}{$-\left[y \log \mathbb{P}(\text{True}\vert \text{s}) + (1-y) \log \mathbb{P}(\text{False}\vert \text{s})\right]$} & \multirow{2}{*}{\cmark} & \multirow{2}{*}{\texttt{[CLS]}} & \multirow{2}{*}{Binary} & \multirow{2}{*}{MC Inference} \\
%         & b) & \texttt{[CLS]} The trophy didn't fit into the brown suitcase because suitcase \texttt{[SEP]} was too small. \texttt{[SEP]} & & & & & \\
%         \midrule
%         P-SENT &  & \texttt{[CLS]} The trophy didn't fit into the brown suitcase because trophy \texttt{[SEP]} was too small. \texttt{[SEP]} & $-\left[y \log \mathbb{P}(\text{True}\vert \text{s}) + (1-y) \log \mathbb{P}(\text{False}\vert \text{s})\right]$ & \xmark & \texttt{[CLS]} & Binary & No Span\\
%         \midrule
%         P-SPAN &  & \texttt{[CLS]} The \underline{trophy} didn't fit into the brown suitcase because \underline{it} was too small. \texttt{[SEP]} & $-\left[y \log \mathbb{P}(\text{True}\vert \text{s}) + (1-y) \log \mathbb{P}(\text{False}\vert \text{s})\right]$ & \xmark & \texttt{[CLS]}, \text{PRON}, \text{NP} & Binary & Baseline\\
%         \bottomrule
%     \end{tabular}}
%     \caption{Overview of the formalizations. MC column indicates whether the model uses MC inference. When MC is \cmark, the model predicts positive only if the query NP $\mathbb{P}(\cdot)$ is highest among all candidates. When MC is \xmark, the model predicts positive if $\mathbb{P}(\cdot)$ is greater than 0.5. EMB indicates the which embeddings are used in the model's final layer. In the loss function, $y$ is the index of the correct input when Label is Index and 0 or 1 when Label is Binary. $\delta_{i,j}$ is the Kronecker delta that is 1 when $i=j$ and 0 otherwise. In the MC-MLM input example, the underline marks NPs to predict. For P-SPAN, the underline marks the NP and PRON spans. Component indicates the hypothesis tested by each formalization.}
%     \label{tab:formalizations}
% \end{table*}

\begin{table*}[h]
    \centering
    \resizebox{.99\textwidth}{!}{
    \begin{tabular}{p{.23\textwidth} p{.2\textwidth} p{.5\textwidth}  p{.07\textwidth} l  p{.03\textwidth} p{.07\textwidth}}
        \toprule
        Ablation & Formalization & Input Example & EMB & Loss & MC & Label\\
        \midrule
        \multirow{2}{*}{\shortstack[l]{From RoBERTa\\ \citep{liu2019RoBERTa}\\ All Components}} & \multirow{2}{*}{MC-MLM} & a) \texttt{[CLS]} The \underline{trophy} didn't fit into the brown suitcase because \texttt{[MASK]} was too small. \texttt{[SEP]} & \multirow{2}{*}{\texttt{[MASK]}} & \multirow{2}{*}{$-\sum_i^n \delta_{y,i} \log \mathbb{P}(\text{NP}_i\vert \text{s})/\sum_j^n\mathbb{P}(\text{NP}_j\vert \text{s})$} & \multirow{2}{*}{\cmark} & \multirow{2}{*}{Index} \\
        & & b) \texttt{[CLS]} The trophy didn't fit into the brown \underline{suitcase} because \texttt{[MASK]} was too small. \texttt{[SEP]} & & & & \\
        \midrule
        \multirow{2}{*}{\shortstack[l]{From WinoGrande\\ \citep{sakaguchi2019winogrande}\\ No MLM}} & \\
        & MC-SENT & \multirow{8}{*}{\shortstack[l]{a) \texttt{[CLS]} The trophy didn't fit into the brown suit-\\case because trophy \texttt{[SEP]} was too small. \texttt{[SEP]}\\ b) \texttt{[CLS]} The trophy didn't fit into the brown suit-\\case because suitcase \texttt{[SEP]} was too small. \texttt{[SEP]}}} & \multirow{8}{*}{\texttt{[CLS]}} & $-\sum_i^n \delta_{y,i} \log \mathbb{P}(\text{NP}_i\vert \text{s}_1,\ldots, \text{s}_n)$ & \cmark & Index \\
        
        & \\
        No Softmax & MC-SENT-PAIR & & & $-\sum_i^n \left[y_i \log \mathbb{P}(\text{True}\vert \text{s}_i) + (1-y_i) \log \mathbb{P}(\text{False}\vert \text{s}_i)\right]$ & \cmark & Binary \\
        &\\
        No Paired Training & MC-SENT-PLOSS & & & $-\left[y \log \mathbb{P}(\text{True}\vert \text{s}) + (1-y) \log \mathbb{P}(\text{False}\vert \text{s})\right]$ & \cmark & Binary \\
        &\\
        No MC Evaluation & P-SENT  & & & $-\left[y \log \mathbb{P}(\text{True}\vert \text{s}) + (1-y) \log \mathbb{P}(\text{False}\vert \text{s})\right]$ & \xmark & Binary \\
        &\\
        \midrule
        \multirow{1}{*}{\shortstack[l]{From SuperGLUE\\ \citep{wang2019superglue}\\ Predict from Span}} & P-SPAN  & \texttt{[CLS]} The \underline{trophy} didn't fit into the brown suitcase because \underline{it} was too small. \texttt{[SEP]} & \texttt{[CLS]}, \text{PRON}, \text{NP} & $-\left[y \log \mathbb{P}(\text{True}\vert \text{s}) + (1-y) \log \mathbb{P}(\text{False}\vert \text{s})\right]$ & \xmark & Binary \\
        \bottomrule
    \end{tabular}}
    \caption{Overview of the formalizations. MC column indicates whether the model uses MC inference. When MC is \cmark, the model predicts positive only if the query NP $\mathbb{P}(\cdot)$ is highest among all candidates. When MC is \xmark, the model predicts positive if $\mathbb{P}(\cdot)$ is greater than 0.5. EMB indicates the which embeddings are used in the model's final layer. In the loss function, $y$ is the index of the correct input when Label is Index and 0 or 1 when Label is Binary. $\delta_{i,j}$ is the Kronecker delta that is 1 when $i=j$ and 0 otherwise. In the MC-MLM input example, the underline marks NPs to predict. For P-SPAN, the underline marks the NP and PRON spans. Component indicates the hypothesis tested by each formalization.}
    \label{tab:formalizations}
\end{table*}


\section{Methodology}
\label{sec:method}
%\subsection{Formalizations}
%We investigate the following hypotheses by comparing the performances of different formalizations. 

We use the following formalizations to interpolate between P-SPAN and MC-MLM, isolating components of MC-MLM that contribute to its improved performance. The formalizations differ by the input formatting, loss function used for training, inference with multiple choice, contextual embeddings used by the final layer, and label type.
Table \ref{tab:formalizations} presents an overview of the formalizations. All formalizations use RoBERTa \citep{liu2019RoBERTa} contextual embeddings.

\paragraph{P-SPAN} We follow \citet{wang2019superglue}'s approach with P-SPAN and use RoBERTa embeddings. The model uses the contextual representations from the PRON and NP to generate a span representation. The span representation is then concatenated with the \texttt{[CLS]} embedding and used by a logistic regression classifier to determine whether the input NP reference is correct. We use this formalization as our baseline.

\paragraph{P-SENT} In P-SENT, we follow the input formatting of \citet{sakaguchi2019winogrande} by replacing the pronoun with a NP candidate and marking it with an additional \texttt{[SEP]} token. The following interpolating formalizations use the same formatting. With the change of input formatting, P-SENT removes the potential difficulty of predicting based on a pointwise span window. Instead, the model simply predicts whether the sentence is correct using the \texttt{[CLS]} token embedding.

\paragraph{MC-SENT-PLOSS} MC-SENT-PLOSS first applies P-SENT to all candidate inputs for a given example. The model then compares the logits in an MC fashion during inference. Losses and training are independent for each candidate. We only differ MC-SENT-PLOSS from P-SENT by using MC evaluation. Despite the two models' shared training procedure, MC evaluation may improve performance by allowing the model to use process of elimination rather than independently resolving the pronoun reference.

\paragraph{MC-SENT-PAIR} The first three formalizations train the model using independent inputs with different candidate NPs. In MC-SENT-PAIR, the model aggregates the losses of all candidate inputs to train with paired examples. We refer to this as paired training. Training the model with highly similar query and candidate choices increases the signal-to-noise ratio, making learning easier.

\paragraph{MC-SENT} In MC-SENT-PLOSS and MC-SENT-PAIR, the model directly compares outputs from P-SENT during MC evaluation. By rescaling these outputs using softmax, the model is able to provide larger gradients to uncertain examples with smaller relative margins. We refer to this as scaling. In MC-SENT, the model feeds the contextual representation of each inptus' \texttt{[CLS]} token into a linear layer followed by a softmax. Through this scaling, the model is able to give higher training weight to difficult examples.

\paragraph{MC-MLM} We use an approach similar to \citet{kocijan2019WSCTrick} for MC-MLM. In this formalization, the PRON in the input is first replaced by \texttt{[MASK]}. The model then uses MLM to evaluate $\mathbb{P}(\text{NP}_i\vert s)$: the probability $\text{NP}_i$ should replace \texttt{[MASK]}. The model then uses a softmax and compares these probabilities. By introducing the MLM component, the model may take advantage of RoBERTa's MLM pre-training to boost its performance.

% \subsection{Contributing Components}

% \paragraph{Span is Harder}

% \paragraph{MC Trivializes Predictions}

% \paragraph{Paired Training}

% \paragraph{Scaled Gradients}

% \paragraph{MLM Helps}

% \paragraph{Span is Harder} Making predictions from span windows may be harder. To test this, we compare P-SPAN with \textbf{P-SENT}, which replaces the PRON with the query NP and marks its location with an additional [SEP] token. This is similar to \citet{trinh2018lmWSC} and \citep{sakaguchi2019winogrande}. Rather than evaluating from a span window, the model simply evaluates whether the input sentence is correct.

% \paragraph{Multiple Choice Trivializes the Prediction} When using multiple choice (MC) based formalization, the model may infer the answer by simply eliminating other candidates. We test this by evaluating the outputs of P-SENT models in an MC fashion and compare performance with P-SENT. We call this second model \textbf{MC-SENT-PLOSS}. Both models learn the same information from training and only differ during inference.

% \paragraph{Pairing} Training the model with highly similar query and candidate choices increases the signal-to-noise ratio, making learning easier. We refer to this as pairing. We quantify the benefit of pairing by comparing MC-SENT-PLOSS with \textbf{MC-SENT-PAIR}. MC-SENT-PAIR aggregates losses for query and candidate inputs during training, which we refer to as paired training.

% \paragraph{Scaling} By rescaling model outputs with mechanisms like softmax, the model is able to provide larger gradients to uncertain examples with smaller margins. We refer to this as scaling. We quantify the benefit of scaling by comparing MC-SENT-PAIR with \textbf{MC-SENT}. For MC-SENT, we follow \citet{sakaguchi2019winogrande} and replace the PRON with the query NP and candidate NP. The model then selects the correct sentence with MC.

% \paragraph{MLM is Easier} MC-MLM may take advantage of RoBERTa's MLM pre-training to boost its performance. We compare MC-SENT with MC-MLM to evaluate the benefit of including MLM.

==> writing/related_works.tex <==
\section{Related Works}
\label{sec:related}

Since the introduction of WSC, several datasets have been released to train and evaluate models \citep{sakaguchi2019winogrande}. The original dataset, which we refer to as WSC-273, consists of 273 hand-crafted problems \citep{levesque2011WSC}. SuperGLUE \citep{wang2019superglue} contains a dataset that expands upon the original WSC-273 by including additional pronoun disambiguation problems \citep{morgenstern2016pdp}. The data recasts these problems into binary True/False tasks. For the remainder of our work, we refer to the SuperGLUE dataset as WSC.

\citet{sakaguchi2019winogrande} present a large-scale Winograd-like dataset  called WinoGrande. While similar to WSC, WinoGrande formats its examples as fill-in-the-blank problems. Its default formalization forms inputs by replacing the blank with each NP option and trains the model to choose the correct answer among all inputs. 

\citet{trinh2018lmWSC} first propose the use of neural network language models for WSC-273. They formalize the task by creating sentences with candidate NPs in place of the PRON. Through this approach \citet{trinh2018lmWSC} achieve an accuracy of 63.7\% on WSC-273.

\citet{wang2019superglue} use a similar approach with P-SPAN and BERT \citep{devlin2018BERT} as a baseline for the SuperGLUE challenge. This formalization, inspired by \citet{tenney2019probing}, generates a span representation from the BERT embeddings of the PRON and candidate NP. This span representation is then used by a logistic regression classifier. Through this formalization, BERT achieves 64.3\% accuracy on WSC.

\citet{kocijan2019WSCTrick} also fine-tune BERT, but formalize the task using MC-MLM. They mask the PRON and use BERT for MLM to evaluate the probability of candidate NP reference conditioned on the training sentence. They train their model using a margin loss. \citet{kocijan2019WSCTrick} use this formalization to fine-tune BERT on additional Winograd-like data to achieve 72.5\% accuracy on WSC-273.

Later contextual embedding models like RoBERTa \citep{liu2019RoBERTa} adopt the MC-MLM formalization, but replace the margin loss with a cross entropy loss. Combined with refined pre-training, RoBERTa outperforms BERT and achieves 89.0\%\footnote{Scores are as reported on the SuperGLUE leader board.} on WSC.
